GaPT: Gaussian Process Toolkit for Online Regression with Application to Learning Quadrotor Dynamics

Gaussian Processes (GPs) are expressive models for capturing signal statistics and expressing prediction uncertainty. As a result, the robotics community has gathered interest in leveraging these methods for inference, planning, and control. Unfortunately, despite providing a closed-form inference solution, GPs are non-parametric models that typically scale cubically with the dataset size, hence making them difficult to be used especially on onboard Size, Weight, and Power (SWaP) constrained aerial robots. In addition, the integration of popular libraries with GPs for different kernels is not trivial. In this paper, we propose GaPT, a novel toolkit that converts GPs to their state space form and performs regression in linear time. GaPT is designed to be highly compatible with several optimizers popular in robotics. We thoroughly validate the proposed approach for learning quadrotor dynamics on both single and multiple input GP settings. GaPT accurately captures the system behavior in multiple flight regimes and operating conditions, including those producing highly nonlinear effects such as aerodynamic forces and rotor interactions. Moreover, the results demonstrate the superior computational performance of GaPT compared to a classical GP inference approach on both single and multi-input settings especially when considering large number of data points, enabling real-time regression speed on embedded platforms used on SWaP-constrained aerial robots.

==> Sections/related_works_notes.tex <==
DO NOT INCLUDE JUST FOR OUR OWN REFERNCE ON DOCUMENTS

\begin{itemize}
     \item application GP to robotics \cite{Deisenroth_GP_robotics}
    \item \textbf{Residual Learning}
    \item Online GP-MPC Learning limited to last 30 points \cite{hewing2019cautious}
    \item Data Driven MPC Scaramuzza GP on MPC \cite{Guillem_datadriveMPC}
    \item GPMPC Uncertainty Propogation \cite{Gang2016GPMPC}
        \item STate Space GP online learning with a car in simulation though \cite{park2020gaussian}
    \cite{WangonlineGP2018} Online learning GP barrier function
    \cite{hewing2019cautious}
    \item \textbf{Alternative GP}
    
    \item Fast GP matrix calculations \cite{Sivaram_fastGP_calc}
    \item Fast Big data GP basically inducing points in parallel \cite{DAS201812}
    \item state space GP\cite{solin2016stochastic}
    \item Extension to State SPace GP  \cite{sarkka2013spatiotemporal}
    \item GP logarithmic time Do the State Space GP regression in parallel  \cite{corenflos2022temporal}
    \item Inducing Points using a subset of the dataset \cite{joaquin_unifiyng_view}
    

    
\end{itemize}




\begin{equation}
    \begin{aligned}
              Q(t)&=  a_n \frac{\partial^n f(t)}{\partial t^n}+\cdots+a_1 \frac{\partial f(t)}{\partial t}+a_0 f(t) \\
\frac{\partial \mathbf{f}(\mathbf{x}) }{\partial \mathbf{x}} &=\mathbf{A} \mathbf{f}(\mathbf{x})+\mathbf{L} Q(\mathbf{x}),\\
\mathbf{y} &=\mathbf{H} \mathbf{f}\left( x_{k}\right)+\varepsilon_{k},\\
\mathbf{f}(\mathbf{x})&=\begin{bmatrix}
f(\mathbf{x}_{\ast}) & \frac{\partial  f(\mathbf{x}_{\ast})}{\partial \mathbf{x}} & \cdots &  \frac{\partial ^m f(\mathbf{x}_{\ast})}{\partial  \mathbf{x}^m}
\end{bmatrix}^\top.
\end{aligned}
\label{eq_SSGP_model}
\end{equation}


In order to solve for an appropriate matrix values for $\mathbf{A}$, $\mathbf{H}$, and $\mathbf{L}$, we construct a relationship through the Fourier transform, $\mathcal{F}$ to the original kernel function and spectral power density. Using eq.~(\ref{eqn:bochner}), we are able to solve for a spectral density of our kernel function. Before, we would like to remind the reader on three key properties of fourier transforms and spectral density


where  that corresponds to the square of the absolute value of the Fourier transform of the process. This value is tunable by the user depending on their confidence. Using the following properties, we are able to convert our spectral density solved from Bochner's theorem into a differential equation. For the following equation let $\mathbf{S}(\omega)$ be the spectral density function of a Fourier transform $\mathbf{s}(i\omega)$. It is important to understand that spectral power density is not the same as the frequency function, but it is the difference between the absolute value of a complex number and a complex number. Also let $\mathcal{F}^{-1}$ be the inverse Fourier transform. We can not directly construct the differential equation from a spectral density. The inverse Fourier transform of an actual frequency domain is what creates the differential equation




==> Sections/timing_table.tex <==
\begin{table*}[t]
    \centering
    \caption{\label{tab:laptop_evaluation}}
    \vspace{-0.75em}
    \caption*{\scshape Inference Time [$\SI{}{\second}$]}
    \vspace{-0.3em}
    \begin{tabular}{c r r r r r r r r r r r r}
        \toprule\toprule
        \multirow{3}{*}{Points} &
        \multicolumn{3}{c}{SISO SSGP} &
        \multicolumn{3}{c}{MISO SSGP} &
        \multicolumn{3}{c}{SISO GPT} &
        \multicolumn{3}{c}{MISO GPT}\\
        \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
        & \multicolumn{1}{c}{PER} & \multicolumn{1}{c}{RBF} & \multicolumn{1}{c}{MAT}
        & \multicolumn{1}{c}{PER} & \multicolumn{1}{c}{RBF} & \multicolumn{1}{c}{MAT}
        & \multicolumn{1}{c}{PER} & \multicolumn{1}{c}{RBF} & \multicolumn{1}{c}{MAT}
        & \multicolumn{1}{c}{PER} & \multicolumn{1}{c}{RBF} & \multicolumn{1}{c}{MAT}\\
        \midrule
        $1$ & $0.006$ & $0.004$ & $0.004$ & $0.006$ & $0.003$ & $0.003$ & $0.003$ & $0.006$ & $0.002$ & $0.0039$ & $0.0017$ & $0.002$\\
        $10$ & $0.009$ & $0.006$ & $0.006$ & $0.016$ & $0.013$ & $0.012$ & $0.010$ & $0.009$ & $0.010$ & $0.0191$ & $0.0103$ & $0.012$ \\
        $50$ & $0.014$ & $0.012$  & $0.013$ & $0.280$ & $0.295$ & $0.281$ & $0.070$ & $0.040$ & $0.043$ & $0.0773$ & $0.0440$ & $0.044$ \\
        $200$ & $0.056$ & $0.046$ & $0.048$ & $1.270$ & $1.301$ & $1.222$ & $0.403$ & $0.220$ & $0.237$ & $0.4316$ & $0.2358$ & $0.245$ \\
        $1000$ & $0.340$ & $0.342$& $0.337$ & $10.600$ & $10.434$ & $9.723$ & $11.429$ & $3.594$ & $4.790$ & $59.353$ & $3.9057$ & $11.390$ \\
        $2500$ & $0.895$ & $0.911$ & $0.903$ & $27.310$ & $28.180$ & $26.450$ & $>60$ & $>60$  & $>60$ & $>60$ & $>60$ & $>60$ \\
        $6000$ & $2.762$ & $2.714$ & $2.905$ & $>60$ & $>60$  & $>60$  & $>60$  & $>60$  & $>60$  &  $>60$ & $>60$ & $>60$ \\
        \bottomrule\bottomrule
    \end{tabular}
        \vspace{-2em}
            \label{tab:inference_time}
\end{table*}


==> Sections/xavier_table_temp.tex <==
% \begin{table*}[t]
%     \centering
%     \caption{\label{tab:xavier_evaluation}}
%     \vspace{-0.75em}
%     \caption*{\scshape SISO and MISO on Xavier NX}
%     \vspace{-0.3em}
%     \begin{tabular}{c c c c c c c c c c c c c}
%         \toprule\toprule
%         \multirow{3}{*}{Points} &
%         \multicolumn{6}{c}{Time [$\SI{}{\milli\second}$]} &
%         \multicolumn{6}{c}{RMSE [$\SI{}{\meter\per\second\squared}$]}\\
%         \cmidrule(lr){2-7}\cmidrule(lr){8-13}
%         & \multicolumn{1}{c}{S-PER} & \multicolumn{1}{c}{M-PER} & \multicolumn{1}{c}{S-RBF} & \multicolumn{1}{c}{M-RBF} & \multicolumn{1}{c}{S-MAT} & \multicolumn{1}{c}{M-MAT} & \multicolumn{1}{c}{S-PER} & \multicolumn{1}{c}{M-PER} & \multicolumn{1}{c}{S-RBF} & \multicolumn{1}{c}{M-RBF} & \multicolumn{1}{c}{S-MAT} & \multicolumn{1}{c}{M-MAT}\\
%         \midrule
%         $1$ & 49 &  & 32 &  & 31 &  &  &  &  &  &  & \\
%         $10$ & 51 &  &  37&  & 33 &  &  &  &  &  &  & \\
%         $50$ & 65 &  & 51 &  & 46 &  &  &  &  &  &  & \\
%         $200$ & 119&  & 102 &  & 98 &  &  &  &  &  &  & \\
%         $1000$ &  451&  & 439 &  & 420 &  &  &  &  &  &  & \\
%         $2500$ & 884 &  &  883&  & 836 &  &  &  &  &  &  & \\
%         $6000$ & 1765 &  & 1716 &  & 2316 &  &  &  &  &  &  & \\
%         \bottomrule\bottomrule
%     \end{tabular}
% \end{table*}

%         $10$ & $1.742$ & $1.186$  & $1.311$ & $--$ & $--$ & $--$  \\
%         $50$ & $1.759$ & $0.962$  & $0.92$ & $--$ & $--$ & $--$  \\
%         $200$ & $1.01$ & $0.938$  & $0.832$ & $--$ & $--$ & $--$  \\
%         $1000$ & $0.808$ & $0.857$  & $0.795$ & $--$ & $--$ & $--$ \\
%         $2500$ & $0.790$ & $0.794$  & $0.794$ & $--$ & $--$ & $--$ \\
%         $6000$ & $0.715$ & $0.796$  & $0.795$ & $--$ & $--$ & $--$   \\


\begin{table*}[t]
    \centering
    \vspace{-0.75em}
    \caption*{\scshape Inference Time [$\SI{}{\second \cdot sample}$]}
    \vspace{-0.3em}
    \begin{tabular}{c r r r r r r r r r r r r}
        \toprule\toprule
        \multirow{3}{*}{Points} &
        \multicolumn{3}{c}{SISO SSGP} &
        \multicolumn{3}{c}{MISO SSGP} &
        \multicolumn{3}{c}{SISO GPT} &
        \multicolumn{3}{c}{MISO GPT}\\
        \cmidrule(lr){2-4}\cmidrule(lr){5-7}\cmidrule(lr){8-10}\cmidrule(lr){11-13}
        & \multicolumn{1}{c}{PER} & \multicolumn{1}{c}{RBF} & \multicolumn{1}{c}{MAT}
        & \multicolumn{1}{c}{PER} & \multicolumn{1}{c}{RBF} & \multicolumn{1}{c}{MAT}
        & \multicolumn{1}{c}{PER} & \multicolumn{1}{c}{RBF} & \multicolumn{1}{c}{MAT}
        & \multicolumn{1}{c}{PER} & \multicolumn{1}{c}{RBF} & \multicolumn{1}{c}{MAT}\\
        \midrule
        $1$ & $0.0482$ & $0.0328$ & $0.0310$ &  &  & &$0.01877$ & $0.0133$ & $0.0123$  & $0.0039$ & $0.0017$ & \\
        $10$ & $0.0548$ & $0.0378$ & $0.0371$ &  &   &$0.0984$  & $0.0609$ & $0.0683$  & $0.010$ & $0.0191$ & $0.0103$ &  \\
        $50$ & $0.0804$ & $0.0597$  & $0.0553$ &  &  &$0.4213$  & $0.2595$ & $0.2624$  & $0.043$ & $0.0773$ & $0.0440$ &  \\
        $200$ & $0.1745$ & $0.1421$ & $0.1367$ &  &  &$3.9072$  & $1.6406$ & $3.9752$  & $0.237$ & $0.4316$ & $0.2358$ &  \\
        $1000$ & $0.9672$ & $0.8329$& $0.7667$ &  &  &$81.936$  & $43.223$ & $52.112$  & $4.790$ & $59.353$ & $3.9057$ &  \\
        $2500$ & $2.2584$ & $2.1870$ & $2.1531$ &  & &$>120$    & $>120$   & $>120$    & $>60$  & $>60$ & $>60$ & $>60$ & $>60$ \\
        $6000$ & $7.4322$ & $7.3941$ & $7.3289$ &  & & $>120$   & $>120$   & $>120$    & $>60$  & $>60$  &  $>60$ & $>60$ & $>60$ \\
        \bottomrule\bottomrule
    \end{tabular}
    \label{tab:inference_time}
\end{table*}
